Localized Shape Modelling with Global Coherence: An Inverse Spectral Approach

Many natural shapes have most of their characterizing features concentrated over a few regions in space. For example, humans and animals have distinctive head shapes, while inorganic objects like chairs and airplanes are made of well-localized functional parts with specific geometric features. Often, these features are strongly correlated -- a modification of facial traits in a quadruped should induce changes to the body structure. However, in shape modelling applications, these types of edits are among the hardest ones; they require high precision, but also a global awareness of the entire shape. Even in the deep learning era, obtaining manipulable representations that satisfy such requirements is an open problem posing significant constraints. In this work, we address this problem by defining a data-driven model upon a family of linear operators (variants of the mesh Laplacian), whose spectra capture global and local geometric properties of the shape at hand. Modifications to these spectra are translated to semantically valid deformations of the corresponding surface. By explicitly decoupling the global from the local surface features, our pipeline allows to perform local edits while simultaneously maintaining a global stylistic coherence. We empirically demonstrate how our learning-based model generalizes to shape representations not seen at training time, and we systematically analyze different choices of local operators over diverse shape categories.

==> sections/Results/Tables/RegionsSMAL.tex <==
\begin{table*}[t!]
%\begin{sidewaystable}

\centering
%Model;MSE error;Area error;Metric error;MSE error head;Area error head;Metric error head;MSE error tail;Area error tail;Metric error tail
\resizebox{\textwidth}{!}{
\begin{tabular}{ k C C C C C C C C C C C }
\toprule
  {  Method} &
  {  \begin{tabular}[c]{@{} c@{}} MSE \\($*10^{-6}$)\end{tabular}} &
  {  \footnotesize \begin{tabular}[c]{@{} c@{}} MSE-$\mathcal{H}$ \\($*10^{-6}$)\end{tabular} } &
  { \footnotesize \begin{tabular}[c]{@{} c@{}} MSE-$\mathcal{T}$ \\($*10^{-6}$)\end{tabular}} &
  {  \begin{tabular}[c]{@{} c@{}} ENN \\($*10^{-6}$)\end{tabular}} &
  { \footnotesize  \begin{tabular}[c]{c} \hspace{-0.4cm} EM \textless ENN \end{tabular}} &
  { \begin{tabular}[c]{@{} c@{}} Area  \\($*10^{-2}$)\end{tabular}} &
  {\footnotesize \begin{tabular}[c]{@{} c@{}} Area-$\mathcal{H}$ \\($*10^{-2}$)\end{tabular}} &
  { \footnotesize \begin{tabular}[c]{@{} c@{}} Area-$\mathcal{T}$ \\($*10^{-2}$)\end{tabular}} &
  { \begin{tabular}[c]{@{} c@{}} Metric \\($*10^{-3}$)\end{tabular}} &
  { \footnotesize \begin{tabular}[c]{@{} c@{}} Metric-$\mathcal{H}$ \\($*10^{-3}$)\end{tabular}} &
  { \footnotesize \begin{tabular}[c]{@{} c@{}} Metric-$\mathcal{T}$ \\($*10^{-3}$)\end{tabular}} \\ 
  \midrule[0.09em]
  
  { LBO 30} & 
  \second{ 1.39} &  \second{1.48 } & \second{4.30} & % MSE
  {3.84} & { 80.2\%} &
  \second{1.90} & \second{2.58} & \second{4.25} & % Area
  \second{3.58} & \second{7.40} & \second{23.6} \\ % Metric
  \midrule[0.07em] \midrule[0.07em]
  %LBO30;1.39e-06;1.90e-02;3.58e-03;1.48e-06;2.58e-02;7.40e-03;4.30e-06;4.25e-02;2.36e-02
  
%   { \begin{tabular}[c]{@{} c@{}} PAT_H 15+15\end{tabular}} & 
  {PAT$_H$ 15+15} &
  {\first{1.08}} &  {\first{1.07} } & {\first{3.07}} & % MSE
  {5.47} & { 86.6\%} &
  {\second{1.63}} & {\second{2.12}} & {\second{3.83}} & % Area
  {\second{3.05}} & {\second{5.96}} & {\second{20.3}} \\ % Metric
  \hline
%PAT15+15_head;1.08e-06;1.63e-02;3.05e-03;1.07e-06;2.12e-02;5.96e-03;3.07e-06;3.83e-02;2.03e-02

%   { \begin{tabular}[c]{@{} c@{}} PAT 15+15\\tail\end{tabular}} &
  {PAT$_T$ 15+15} &
  {3.93} &  {4.20 } & {11.5} & % MSE
  {11} & { 64.6\%} &
  {3.05} & {4.03} & {6.26} & % Area
  {6.13} & {14.1} & {36.9} \\ % Metric 
  %PAT15+15_tail;3.93e-06;3.05e-02;6.13e-03;4.20e-06;4.03e-02;1.41e-02;1.15e-05;6.26e-02;3.69e-02
  \midrule[0.13em]
  
%   { \begin{tabular}[c]{@{} c@{}} PAT10+10+10\\head tail\end{tabular}} & 
  {PAT$_{H+T}$ 10+10+10} &
  {1.96} &  {2.01} & {6.08} & % MSE
  {7.02} & { 75.8\%} &
  {2.37} & {3.07} & {5.16} & % Area
  {4.48} & {9.53} & {29.4} \\ % Metric
  \hline
  %1.96e-06;2.37e-02;4.48e-03;2.01e-06;3.07e-02;9.53e-03;6.08e-06;5.16e-02;2.94e-02
  
    % { \begin{tabular}[c]{@{} c@{}} PAT15+10+5\\head tail\end{tabular}} & 
    {PAT$_{H+T}$ 15+10+5} &
  \third{1.82} &  \third{1.88} & \third{5.66} & % MSE
  {6.54} & { 79.8\%} &
  \third{2.24} & \third{2.90} & \third{5.01} & % Area
  \third{4.18} & \third{8.48} & \third{28.6} \\ % Metric
  % PAT15+10+5_head_tail
 
\bottomrule
\end{tabular}}
\caption{Reconstruction error on the SMAL test set with various regions.
For each column, we highlighted the top three results in red with decreasing intensity.}
\label{tab:errorsRegionsSMAL}
%\end{sidewaystable}
\end{table*}


==> sections/Results/Tables/RegionsSURREAL.tex <==
\begin{table*}[t!]
\centering
\footnotesize
%\resizebox{0.7\textwidth}{!}{
\begin{tabular}{ k C C C C C }
\toprule
  {  Method} &
  {  \begin{tabular}[c]{c} MSE \\ ($*10^{-6}$)\end{tabular}} & 
  %{  \begin{tabular}[c]{c} MSE-$\subX$ \\ ($*10^{-6}$) \end{tabular}} & 
  %{  \begin{tabular}[c]{c} MSE-$\subX^C$ \\ ($*10^{-6}$) \end{tabular}} &
  {  \begin{tabular}[c]{c} ENN \\ ($*10^{-6}$) \end{tabular}} & 
  { \begin{tabular}[c]{c} \hspace{-0.4cm} EM \textless ENN \end{tabular}} &
  { \begin{tabular}[c]{@{} c@{}} Area \\ ($*10^{-3}$)\end{tabular}} &
  %{ \begin{tabular}[c]{@{} c@{}} Area-$\subX$ \\ ($*10^{-3}$)\end{tabular}} &
  { \begin{tabular}[c]{@{} c@{}} Metric  \\ ($*10^{-3}$)\end{tabular}} 
  %{ \begin{tabular}[c]{@{} c@{}} Metric-$\subX$ \\ ($*10^{-3}$)\end{tabular}}\\
  \\
  \midrule[0.09em]

  {  \begin{tabular}[c]{@{} c@{}}LBO 30\end{tabular}} &
  {  1.7} & %{  2.12} & {  1.61} &
  {  15.4} & {  99.57\%} &
  {8.19} & %{10.1} & 
  {2.62} %& {5.23}
  \\ 
  \midrule[0.07em] \midrule[0.07em] 
% LBO30;8.19e-03;2.62e-03;1.11e-07;1.01e-02;5.23e-03

  {  PAT$_H$ 15+15 } &
  {  \second{0.71}} &%  { \first{0.5}} &  \second{ 0.76} &
  {  39.1} &  {  {100\%}} &
  {\first{4.58}} & %{\first{4.94}} & 
  {\second{1.81}} %& \second{2.27}
  \\ \midrule[0.07em] \midrule[0.07em]
%PAT15+15;4.58e-03;1.81e-03;2.42e-08;4.94e-03;2.27e-03

  { PAT$_F$ 15+15} &
  { 4.33 } &  %{ } &  { } &
  {86.3} &  {  {98.7\%}} &
  {13} & %{} & 
  {4.98} %& \second{}
  \\ \hline
  
  { PAT$_T$ 15+15} &
  { 1.71} &  %{ } &  { } &
  {48.6} &  {  {100\%}} &
  {9.35} & %{} & 
  {2.96} %& \second{}
  \\ 
  \midrule[0.07em] \midrule[0.07em]

  { PAT$_{H+T}$ 10+10+10} &
  \third{ 0.89 } & % { } &  { } &
  {74.6} &  {  {99.57\%}} &
  \third{5.61} & %{} & 
  \third{1.98} %& \second{}
  \\ 
  \hline
  
    { PAT$_{H+T}$ 15+15+15} &
    \first{ 0.68 } & % { } &  { } &
  {48.1} &  {  {100\%}} &
  {\second{4.86}} & %{} & 
  \first{1.78} %& \second{}
  \\ 

\bottomrule
\end{tabular}
%}
\caption{Reconstruction error on SURREAL test set considering various regions. For each column, we highlighted the top three results in red with decreasing intensity.} 
\label{tab:regionsSURREAL}
\end{table*}

==> sections/implementation.tex <==
\section{Implementation details}
\label{sec:details}

\subsection{Data preprocessing.} 

\subsection{Network hyperparameters.} 

\subsection{Timing and complexity.} 

==> tabBaloon.tex <==
\begin{table*}[]
\centering
\begin{tabular}{ c| c |c| c| c| c| c| c| c| c }
\toprule
  {  Method} &
  {  MSE} &
  {  \begin{tabular}[c]{@{} c@{}} MSE \\ Region\end{tabular} } &
  {  \begin{tabular}[c]{@{} c@{}} MSE \\ Out Region\end{tabular}} &
  {  \begin{tabular}[c]{@{} c@{}} NN \\ error \end{tabular}} &
  {  Err\_model \textless err\_nn} & 
  {\begin{tabular}[c]{@{} c@{}} Area \\ error \end{tabular}} &
  {\begin{tabular}[c]{@{} c@{}} Metric \\ error \end{tabular}} &
  {\begin{tabular}[c]{@{} c@{}} Align \\ error \end{tabular}} \\ \midrule[0.09em]
  
  {  \begin{tabular}[c]{@{} c@{}}LBO 30\end{tabular}} &
  {   7.28} &
  {  34.1} &
  {  1.91} &
  {  57.9} &
  {  57.71\%} &
  {5.94} &
  {2740} &
  {30.2} \\ \midrule[0.07em] \midrule[0.07em]

  {  \begin{tabular}[c]{@{} c@{}}PAT 20+10\end{tabular}} &
  {  39.4} &
  {  86.7} &
  {  29.9} &
  {  145} &
  {  27.36\%} & 
  {10.1} &
  {7710} &
  {64.7} \\ \hline
   \midrule[0.07em] \midrule[0.07em]
  
\bottomrule
\end{tabular}
\caption{Reconstruction error on the Baloon dataset. All the numbers should be multiplied by 10e-6}
\label{tab:errorsBaloon}
\end{table*}

==> tabCUBE.tex <==
\begin{table*}[t!]
\footnotesize
\centering

\begin{tabular}{ k C C C C C C C C C C C }
\toprule
  {  Method} &
  {  MSE} &
  {  \begin{tabular}[c]{@{} c@{}} MSE-$\subX$\end{tabular} } &
  {  \begin{tabular}[c]{@{} c@{}} MSE-$\subX^C$\end{tabular}} &
  {  \begin{tabular}[c]{@{} c@{}} ENN \end{tabular}} &
  {  \begin{tabular}[c]{c} \hspace{-0.4cm} EM \textless ENN \end{tabular}} &
  { \begin{tabular}[c]{@{} c@{}} Area  \\($*10^4$)\end{tabular}} &
  { \begin{tabular}[c]{@{} c@{}} Metric \\($*10^3$)\end{tabular}} &
  { \begin{tabular}[c]{@{} c@{}} Align \end{tabular}} &
  { \begin{tabular}[c]{@{} c@{}} Area-$\subX$ \\($*10^4$)\end{tabular}} &
  { \begin{tabular}[c]{@{} c@{}} Metric-$\subX$ \\($*10^4$)\end{tabular}} \\ 
  \midrule[0.09em]
  
  { LBO 30} & { 11} &  { 62.5} & { 0.65} &
  {15} & { 60\%} &
  {1.96} & {6.63} & {60.3} &
  {6.80} & {3.38} \\ \hline
  %LBO30;1.96e-02;6.63e-03;6.03e-05;6.80e-02;3.38e-02

    { LBO 50} &
  {10.7} &  { 62} & \second{ 0.45}  &
  {15} & { 65\%}  &
  {1.80} &  {6.41} & {60.2} &
  {6.76} & {3.33}  \\ \hline
%LBO50;1.80e-02;6.41e-03;6.02e-05;6.76e-02;3.33e-02

  { LBO 80} & { 11.1} &  { 63.5} & { 0.63} &
  { 14}  & { 61\%}  &
  {1.73} & {6.54} & {61.1} &
  {6.59} & {3.37}  \\ \midrule[0.07em] \midrule[0.07em]
  %LBO80;1.73e-02;6.54e-03;6.11e-05;6.59e-02;3.37e-02

  { PAT 20+10} & { 6.65} & { 37.8} & { \first{0.42}} &  
  {309} & { 88\%} &
  {1.78} & {4.81} & {37} &
  {6.25} & {2.42}  \\ \hline 
  %PAT20+10;1.78e-02;4.81e-03;3.70e-05;6.25e-02;2.42e-02
  
  { PAT 15+15} & { 5.66} & { 27.1} & { 1.36}  &
  {1090} & { 95\%} &
  {2.31} & {3.96} & {25.5} &
  {6.01} & {1.75}  \\ \hline
  %PAT15+15;2.31e-02;3.96e-03;2.55e-05;6.01e-02;1.75e-02

  { PAT 10+20} & { 4.91} & { 26.3} & { 0.63} &
  {1720}  & {100\%} &
  \third{1.43} & {3.59} & {24.7} &
  {5.37} & {1.79}  \\ \midrule[0.13em]
  %PAT10+20;1.43e-02;3.59e-03;2.47e-05;5.37e-02;1.79e-02
  
  { PAT 40+10} & { 6.76} & { 38.5} & \first{ 0.42}  &
  {79} & { 86\%} &
  {1.59} & {4.89} & {37.6} &
  {6.13} & {2.49}  \\ \hline
  %PAT40+10;1.59e-02;4.89e-03;3.76e-05;6.13e-02;2.49e-02

  { PAT 25+25} &
  { \first{3.59} } &  \second{ 19.1} &  \third{ 0.5}  &
  {2060} &  {100\%} & 
  {\first{1.33}} & {\first{2.76}} & \third{18.1} &
  \second{4.52} & \third{1.39}  \\ \hline 
  %PAT25+25;1.33e-02;2.76e-03;1.81e-05;4.52e-02;1.39e-02

  { PAT 10+40} &
  { 6.70} & { 23.4} & { 3.36} & 
  {1860} & {  100\%} &
  {1.51} & {3.63} & \second{16.9} &
  {4.62} & \second{1.32}  \\ \midrule[0.13em]
%PAT10+40;1.51e-02;3.63e-03;1.69e-05;4.62e-02;1.32e-02
    
  { PAT 40+40} &
  { \second{3.77}} &  { \first{18.3}} & { 0.85} & 
  {2310} & { 100\%} &
  \second{1.35} & \second{2.84} & {\first{16.3}}  &
  {\first{4.44}} & {\first{1.28}} \\
  %PAT40+40;1.35e-02;2.84e-03;1.63e-05;4.44e-02;1.28e-02

  \midrule[0.07em] \midrule[0.07em]
    
  { HAM 25+25 } & { \third{4.07}} & \third{ 20.1} & { 0.86}  &
  {2050} & { 99\%} &
  {\first{1.33}} & \third{3.05} &  {18.4} &
  \third{4.56} & {1.41}  \\ \midrule[0.07em] \midrule[0.07em]
    %HAM25+25;1.33e-02;3.05e-03;1.84e-05;4.56e-02;1.41e-02

  { LMH 25+25 } & { 14.7} & { 69.2} & { 3.81} &
  {137}  & { 65\%} &
  {1.96} & {6.08} & {59.6}  &
  {6.85} & {2.77} \\
  %LMH25+25;1.96e-02;6.08e-03;5.96e-05;6.85e-02;2.77e-02

 
\bottomrule
\end{tabular}
\caption{Reconstruction error on the CUBE dataset. All the numbers should be multiplied by 1e-6. For each column, we highlighted the top three results in red with decreasing intensity.}
\label{tab:errorsTOY}
\end{table*}

==> tabSURREAL.tex <==


\begin{table*}[t!]
\centering
\footnotesize
\begin{tabular}{ k C C C C C C C C C C C}
\toprule
  {  Method} & {  MSE} & 
  {  \begin{tabular}[c]{c} MSE-$\subX$\end{tabular}} & 
  {  \begin{tabular}[c]{c} MSE-$\subX^C$\end{tabular}} &
  {  \begin{tabular}[c]{c} ENN \end{tabular}} & 
  { \begin{tabular}[c]{c} \hspace{-0.4cm} EM \textless ENN \end{tabular}} &
  { \begin{tabular}[c]{@{} c@{}} Area \\ ($*10^3$)\end{tabular}} &
  { \begin{tabular}[c]{@{} c@{}} Metric  \\ ($*10^3$)\end{tabular}} &
  { \begin{tabular}[c]{@{} c@{}} Align \\ ($*10^{-2}$)\end{tabular}}&
  { \begin{tabular}[c]{@{} c@{}} Area-$\subX$ \\ ($*10^3$)\end{tabular}} &
  { \begin{tabular}[c]{@{} c@{}} Metric-$\subX$ \\ ($*10^3$)\end{tabular}}\\
  \midrule[0.09em]

  {  \begin{tabular}[c]{@{} c@{}}LBO 30\end{tabular}} &
  {  1.7} & {  2.12} & {  1.61} &
  {  15.4} & {  99.57\%} &
  {8.19} & {2.62} & {11} & {10.1} & {5.23}\\ \midrule[0.07em] \midrule[0.07em] 
% LBO30;8.19e-03;2.62e-03;1.11e-07;1.01e-02;5.23e-03

  {  \begin{tabular}[c]{@{} c@{}}PAT 25+5\end{tabular}} &
  {  1.1} &  {  1.42} & {  1.03} &
  {  19.6} & {  {100\%}} &
  {15} & {2.21} & {4.8} & {23.9} & {3.32}\\ \hline
% PAT25+5;1.50e-02;e-03;4.80e-08;2.39e-02;3.32e-03

  {  \begin{tabular}[c]{@{} c@{}}PAT 20+10\end{tabular}} & 
  \third{  0.77} & {0.75} & \third{ 0.77} & 
  {  28.8} &  {  { 100\%}} &
  {5.24} & {1.87} & {\first{2.28}} & \second{5.09} & {\first{2.25}}\\ \hline
%PAT20+10;5.24e-03;1.87e-03;2.28e-08;5.09e-03;2.25e-03

  {  \begin{tabular}[c]{@{} c@{}}PAT 15+15\end{tabular}} &
  {  \first{0.71}} &  { \first{0.5}} &  \second{ 0.76} &
  {  39.1} &  {  {100\%}} &
  {\first{4.58}} & {\first{1.81}} & {2.42} & {\first{4.94}} & \second{2.27}\\ \midrule[0.07em] \midrule[0.07em]
%PAT15+15;4.58e-03;1.81e-03;2.42e-08;4.94e-03;2.27e-03

  {  \begin{tabular}[c]{@{} c@{}}HAM 25+5\end{tabular}} &
  {  0.98} & {  1.13} & { 0.95} &  { 19} &  {  { 100\%}} &
  {5.33} & \third{1.93} & {3.18} & {5.65} & {2.47}\\ \hline
  %HAM25+5;5.33e-03;1.93e-03;3.18e-08;5.65e-03;2.47e-03

  {  \begin{tabular}[c]{@{} c@{}}HAM 20+10\end{tabular}} &
  \second{  0.73}& \third{  0.67} & {  \textbf{0.75}} &
  {  27.4} &  {  { 100\%}} &
  \third{5.11} & \second{1.86} & {2.43} & \second{5.09} & \third{2.29}\\ \hline
%HAM20+10;5.11e-03;1.86e-03;2.43e-08;5.09e-03;2.29e-03

  {  \begin{tabular}[c]{@{} c@{}}HAM 15+15\end{tabular}} &
  {  0.86} & \second{ 0.57} & { 0.92} &
  {  38.9} & { { 100\%}} &
  \second{5.10} & {2.11} & \second{2.36} & \third{5.21} & {2.37}\\ \midrule[0.07em] \midrule[0.07em]
% HAM15+15;5.10e-03;2.11e-03;2.36e-08;5.21e-03;2.37e-03

  {  \begin{tabular}[c]{@{} c@{}}LMH 25+5\end{tabular}} &
  { 2.7} & {  2.49} & {  2.75} &
  {  29.9} &  {  { 100\%}} &
  {10.6} & {3.37} & {14} & {11.7} & {5.71}\\ \hline
%LMH25+5;1.06e-02;3.37e-03;1.40e-07;1.17e-02;5.71e-03
  {  \begin{tabular}[c]{@{} c@{}}LMH 20+10\end{tabular}} &
  { 2.4} & { 2.06} &  { 2.47} &
  { 32.5} & { { 100\%}} &
  {9.64} & {3.26} & {8.52} & {8.62} & {3.97}\\ \hline
%LMH20+10;9.64e-03;3.26e-03;8.52e-08;8.62e-03;3.97e-03
  {  \begin{tabular}[c]{@{} c@{}}LMH 15+15\end{tabular}} &
  {  1.5} &  { 0.98} & {  1.61} &
  {  31.2} & { { 100\%}} &
  {7.15} & {2.62} & {3.96} & {6.16} & {2.67}\\ \midrule[0.07em] \midrule[0.07em]
  %LMH15+15;7.15e-03;2.62e-03;3.96e-08;6.16e-03;2.67e-03

{ \begin{tabular}[c]{@{} c@{}}\cite{instant2020} PAT 15+15\end{tabular}} & {3.1} & {3.89} & {2.92} & 51.3 & { 100\%} & 19.81 & 4.46 & 19.37 & 32.93 & 8.44 \\  \hline
{\begin{tabular}[c]{@{} c@{}}\cite{instant2020}$_{big}$ PAT 15+15\end{tabular}} & {2.51} & {1.8} & {2.67} & 51.3 & { 100\%} & 16.9 & 4.52 & 19.20 & 22.25 & 9.28 \\ \hline
{ \begin{tabular}[c]{@{} c@{}}\cite{instant2020}$_{big}$ LBO 30\end{tabular}} & {2.51} & {2.26} & {2.56} &  15.09 & 99.96\%   & 15.74 & 4.35 & 15.26 & 22.87 & 7.24 \\

\bottomrule
\end{tabular}
\caption{Reconstruction error on the SURREAL dataset. All the numbers should be multiplied by 1e-6. For each column, we highlighted the top three results in red with decreasing intensity.}
\label{tab:errorsSURREAL}
\end{table*}

==> tabTOY.tex <==
\begin{table*}[]
\centering

\begin{tabular}{ c| c |c| c| c| c| c| c| c| c }
\toprule
  {  Method} &
  {  MSE} &
  {  \begin{tabular}[c]{@{} c@{}} MSE-R \end{tabular} } &
  {  \begin{tabular}[c]{@{} c@{}} MSE-OR \\ Out Region\end{tabular}} &
  {  \begin{tabular}[c]{@{} c@{}} ENN \\ error \end{tabular}} &
  {  EM \textless ENN} & 
  { \begin{tabular}[c]{@{} c@{}} Area  \end{tabular}} &
  { \begin{tabular}[c]{@{} c@{}} Metric \end{tabular}} &
  { \begin{tabular}[c]{@{} c@{}} Align \end{tabular}} \\ \midrule[0.09em]
  
  {  LBO 50} &
  {  20.3} &
  {  47.2} &
  {  14.9} &
%  {  \textbf{1.57e-02}} &
  {  122} &
  {  47.71\%} &
  {} &
  {} &
  {} \\ \hline
  
  {  LBO 30} &
  {  4.21} &
  {  18.6} &
  {  1.34} &
%  {  \textbf{1.57e-02}} &
  {  137} &
  {  42.48\%}  &
  {9.19} &
  {3260} &
  {15.5} \\ \hline
  
  {  LBO 30Bias} &
  { 6.04 } &
  { 21.6 } &
  { 2.92 } &
  { 137 } &
  { 49.67\%}  & 
  {7.3} &
  {3000} &
  {16.7} \\ \midrule[0.07em] \midrule[0.07em]

  {  PAT 20+10} &
  {  \textbf{2.01}} &
  {  \textbf{9.81}} &
  {  \textbf{0.445}} &
%  {  1.61e-02} &
  {  142} &
  {  \textbf{63.4\%}}  &
  { \textbf{6.83}} &
  { \textbf{1840}} &
  { \textbf{9.05}} \\ \hline
  
  { PAT 20+10Bias} &
  { 52.2 } &
  { 58.6 } &
  { 51 } &
  { 142 } &
  {  41.83\%}  &
  {7.27} &
  {3290} &
  {9.23} \\ \hline

  {  PAT 15+15} &
  {  2.30} &
  {  10.3} &
  {  0.702} &
%  {  1.58e-02} &
  {  \textbf{131}} &
  {  45.1\%}  &
  {} &
  {} &
  {} \\ \hline

    {  PAT 0+15} &
  {  9460 } &
  { 16800 } &
  { 7990 } &
%  {  1.58e-02} &
  { 11500} &
  {  58.82\%}  &
  {212} &
  {138000} &
  {10.1} \\ \hline

  {  PAT 40+15} &
  { 3.26 } &
  { 13.1 } &
  { 1.29 } &
%  {  1.58e-02} &
  { 164 } &
  {  41.18\%}  &
  {} &
  {} &
  {} \\ \hline
  
    {  \begin{tabular}[c]{@{} c@{}}PAT 20+30\end{tabular}} &
  { 5.02 } &
  { 14.2 } &
  { 3.17 } &
%  {  1.58e-02} &
  { 153 } &
  {  26.08\%}  &
  {} &
  {} &
  {} \\ \hline
  
  {  \begin{tabular}[c]{@{} c@{}}PAT 20+10 localDist\end{tabular}} &
  {  3.31} &
  {  12.3} &
  {  1.50} &
%  {  1.58e-02} &
  {  142} &
  {  46\%}  &
  {} &
  {} &
  {} \\ \midrule[0.07em] \midrule[0.07em]
  
\bottomrule
\end{tabular}
\caption{Reconstruction error on the TOY dataset. All the numbers should be multiplied by 10e-6}
\label{tab:errorsTOY}
\end{table*}
